FiLM-Ensemble: Probabilistic Deep Learning via Feature-wise Linear Modulation

The ability to estimate epistemic uncertainty is often crucial when deploying machine learning in the real world, but modern methods often produce overconfident, uncalibrated uncertainty predictions. A common approach to quantify epistemic uncertainty, usable across a wide class of prediction models, is to train a model ensemble. In a naive implementation, the ensemble approach has high computational cost and high memory demand. This challenges in particular modern deep learning, where even a single deep network is already demanding in terms of compute and memory, and has given rise to a number of attempts to emulate the model ensemble without actually instantiating separate ensemble members. We introduce FiLM-Ensemble, a deep, implicit ensemble method based on the concept of Feature-wise Linear Modulation (FiLM). That technique was originally developed for multi-task learning, with the aim of decoupling different tasks. We show that the idea can be extended to uncertainty quantification: by modulating the network activations of a single deep network with FiLM, one obtains a model ensemble with high diversity, and consequently well-calibrated estimates of epistemic uncertainty, with low computational overhead in comparison. Empirically, FiLM-Ensemble outperforms other implicit ensemble methods, and it and comes very close to the upper bound of an explicit ensemble of networks (sometimes even beating it), at a fraction of the memory cost.

==> chapters/04_background.tex <==
\section{Background: Feature-wise Linear Modulation (FiLM)} \label{sec:background_film}

The concept of Feature-wise Linear Modulation was originally proposed by Perez \textit{et al.} as a way to improve the visual reasoning capabilities of neural networks by computing adaptive normalization parameters from conditioning information~\citep{perez2018film}. As such, FiLM can be seen as a generalization of conditional normalization \textcolor{red}{TODO CITE}. This was initially done to allow CNNs to adaptively process feature maps for visual question answering, using the questions as conditioning information. In \citet{perez2018film}, the questions were processed using an RNN to produce \emph{FiLM parameters}, which then modulated the layers of a CNN. This achieved excellent results without resorting to attention mechanisms or other advanced methods.

In its general form, FiLM uses two functions $f_c$ and $h_c$ to compute feature normalization parameters 
% $\gamma_{i,c} = f_c(\mathbf{x}_i)$ and $\beta_{i,c} = h_c(\mathbf{x}_i)$
%
\begin{equation}
    \gamma_{i,c} = f_c(\mathbf{x}_i)
\end{equation}
and
\begin{equation}
  \beta_{i,c} = h_c(\mathbf{x}_i)
\end{equation}
%
based on conditioning information $\mathbf{x}_i$, where $i$ denotes the input's index and $c$ denotes the feature map's index. $\mathbf{x}_i$ is generally not the same input given to the conditioned network, but that is not a requirement. In practice, $f_c$ and $h_c$ are often combined into a single function since sharing parameters makes this step more efficient.

In the modulated network, features are transformed using an affine operation using the associated normalization parameters calculated by the FiLM network:
\begin{equation}
    \textrm{FiLM}(\mathbf{F}_{i,c}|\gamma_{i,c}, \beta_{i,c}) = \gamma_{i,c} \mathbf{F}_{i,c} + \beta_{i,c}.
\end{equation}
This operation is similar to other normalization layers and can be learned in an end-to-end manner with little computational overhead and incurring in only a small increase in the number of learnable parameters.



Such feature modulation allows for a single network to perform different operations based on the conditioning information. Feature maps can be scaled, inverted, or disabled depending on the FiLM parameters. It generalizes the operations used for batch normalization and dropout, although in the latter case it lacks stochasticity. Similarly to dropout, each modulation can be seen as a sub-network, but where elements are not only enabled or disabled in a binary way, but instead are combined in different ways to achieve different results. 
%


==> checklist.tex <==
\section*{Checklist}

% fixed - these macros did not exist in the 2020 style file that you previously used
%\ozgur{why do we have error with this? answerYes or answerNo doesnt appear}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
    {\bf Purely methodological contribution that, when added to a learning system, does not alter its potential societal impacts. If anything, better uncertainty calibration reduces the risk of negative effects caused by undetected prediction errors.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
    {\bf license information for the used datasets is public.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> tables/cifar10.tex <==
\begin{table}
  \caption{Cifar10/VGG-11 performance comparison. The best score for each metric is printed \textbf{bold}.}
  \label{t:cifar10}
  \centering
  \begin{tabular}{lcccccc}
    \toprule
    %\multicolumn{2}{c}{Part}                   \\
   % \cmidrule(r){1-2}
    Method    & Acc ($\uparrow$) & ECE ($\downarrow$)  & Entropy ($\downarrow$)  & AUROC ($\uparrow$)   & Disagr ($\uparrow$)  & KL-div ($\uparrow$)  \\
    \midrule
    Single Network  & x  & x  & x  & x  & x  & x  \\
    Deep Ensemble   & x  & x  & x  & x  & x  & x  \\ \midrule
    MC-Dropout      & x  & x  & x  & x  & x  & x \\
    BatchEnsemble  & x  & x  & x  & x  & x  & x \\
    MIMO            & x  & x  & x  & x  & x  & x \\
    Masksemble  & x  & x  & x  & x  & x  & x  \\
    FiLM-Ensemble  & x  & x  & x  & x  & x  & x  \\

    \bottomrule
  \end{tabular}
\end{table}




==> tables/genome.tex <==
\begin{table}
  \caption{Performance comparison for 6mA Identification dataset. $g$ is the initialization gain factor for FiLM-Ensemble. Tuning $g$ allows trade-off between accuracy and calibration. The best score for each metric is printed in \textbf{bold}, the second best is \underline{underlined}.}
  \label{t:deep6ma}
  \centering
  \begin{tabular}{l|ccc|cccc}
    \toprule

   % \cmidrule(r){1-2}
       Method    & \multicolumn{3}{c}{Accuracy (\%)  ($\uparrow$)} & \multicolumn{3}{|c}{ECE  ($\downarrow$)}                  \\
        \midrule

      \# member  & 2 & 4 & 8 & 2    & 4 & 8   \\
    \midrule
    Single & 93.67 & 93.67 & 93.67 & 0.0247 & 0.0247   & 0.0247  \\
    Deep Ensemble   & 93.73  & \textbf{93.77}  & \textbf{93.78} & 0.0257 & 0.0262  & 0.0266  \\
    MIMO & 93.22 & 91.81& 83.48 & 0.0413 & 0.0561 & 0.0183\\
    BatchEnsemble & 91.42 & 91.11 & 85.54 & 0.0386 & 0.0551 & 0.0838\\ 
    %MC-Dropout & 93.74 & +93.93 & ++93.99 & 0.0037 & ++0.0023 & +0.0030\\
    FiLM-Ensemble ($g=4$)  &  \underline{93.81} &  \underline{93.76} &  \textbf{93.78}  & 0.0269 & 0.0278 & 0.0266   \\
    FiLM-Ensemble ($g=8$)  &  \textbf{93.89} &  \underline{93.76} &  \underline{93.76}  & 0.0239 & 0.0230 & 0.0265   \\
    FiLM-Ensemble ($g=16$)  &  93.77 &  93.74 &  93.73  & \underline{0.0195} & \underline{0.0182} & \underline{0.0175}   \\
    FiLM-Ensemble ($g=32$)  &  93.67 &  93.66 &  93.64  & \textbf{0.0144} & \textbf{0.0162} & \textbf{0.0112}   \\
    

    \bottomrule
  \end{tabular}
\end{table}


